Collaborative Manipulation of Deformable Objects with Predictive Obstacle Avoidance

Manipulating deformable objects arises in daily life and numerous applications. Despite phenomenal advances in industrial robotics, manipulation of deformable objects remains mostly a manual task. This is because of the high number of internal degrees of freedom and the complexity of predicting its motion. In this paper, we apply the computationally efficient position-based dynamics method to predict object motion and distance to obstacles. This distance is incorporated in a control barrier function for the resolved motion kinematic control for one or more robots to adjust their motion to avoid colliding with the obstacles. The controller has been applied in simulations to 1D and 2D deformable objects with varying numbers of assistant agents, demonstrating its versatility across different object types and multi-agent systems. Results indicate the feasibility of real-time collision avoidance through deformable object simulation, minimizing path tracking error while maintaining a predefined minimum distance from obstacles and preventing overstretching of the deformable object. The implementation is performed in ROS, allowing ready portability to different applications.

==> 98_acknowledgment/ack.tex <==
\section*{ACKNOWLEDGMENT}
% aaaaa aaaaaaa aaaaa aaaaaaaaaa aaaa a aaaa aaa aaaa aaaaaa aaaaaaa aaaaaaaaa aaaaaaa aaaaa aaaaaa aa aaaaaaaaa
